AdaptEx: A Self-Service Contextual Bandit Platform

This paper presents AdaptEx, a self-service contextual bandit platform widely used at Expedia Group, that leverages multi-armed bandit algorithms to personalize user experiences at scale. AdaptEx considers the unique context of each visitor to select the optimal variants and learns quickly from every interaction they make. It offers a powerful solution to improve user experiences while minimizing the costs and time associated with traditional testing methods. The platform unlocks the ability to iterate towards optimal product solutions quickly, even in ever-changing content and continuous "cold start" situations gracefully.

==> SECTIONS/bios.tex <==
\section{Author Biographies}\label{sec:bios}

\textbf{William Black} is a scientist in the RL Team at Expedia Group. He holds a Masters in Mathematics and ML from the University of Oxford.
\\
\textbf{Ercument Ilhan} is a scientist in the RL team at Expedia Group. He obtained his PhD from Queen Mary University of London where he worked on Deep Reinforcement Learning. 
\\
\textbf{Andrea Marchini} is a senior scientist at Expedia Group where he develops RL algorithms. Previously he worked in applied machine learning across various industries. He holds a PhD in Physics from Sapienza University of Rome.
\\
\textbf{Vilda Markeviciute} is a ML scientist in the RL team at Expedia Group. She holds a PhD in Applied Maths from University of Cambridge.

==> SECTIONS/related_work.tex <==
\section{RELATED WORK}



% Several industry platforms have emerged for deploying contextual bandits to optimize user experiences. Microsoft Personalizer (MP) is a fully managed cloud service that provides contextual bandit for applications to optimize user experiences. It is built on the Vowpal Wabbit\footnote{\text{See more:\,}\mbox{\url{https://vowpalwabbit.org/index.html}}} machine learning framework to enable scalable and low-latency training. MP allows configuring hyperparameters like exploration percentage, learning policy and reward aggregation. In term of exploration strategy it currently uses epsilon greedy to explore while AdaptEx supports a wider variety varienty of eeploration algorithms (See \ref{sec:algos}).

% Amazon Personalize offers a managed bandit service but with limited algorithm options compared to Personalizer [5]. It lacks advanced configurability though may be easier to implement. Optimizely Rollouts focuses on basic A/B testing rather than robust contextual learning [6].


% Microsoft Personalizer provides a fully managed bandit service, simplifying implementation through their cloud infrastructure [14]. It leverages the Vowpal Wabbit machine learning framework to enable scalability and low latency algorithm implementations [16]. However, it offers less flexibility compared to AdaptEx in terms of customizing algorithms and rewards. Amazon Personalize is part of their broader machine learning platform, but only supports basic random exploration algorithms [1]. Optimizely Rollouts enables easy A/B testing through their intuitive interface, but lacks more advanced bandit algorithms and large-scale personalization [11].

% Compared to these existing industry platforms, a key advantage of AdaptEx is being a self-service platform that provides accessibility for non-experts to deploy contextual bandits. It combines this with advanced algorithms, custom rewards tuned to business metrics, and scalability to millions of options. The platform's ability to handle cold starts and new content situations also differentiates it. Overall, AdaptEx delivers an industry-leading balance of ease-of-use, flexibility, and contextual personalization capabilities.
